TTK is Getting MPI-Ready

This system paper documents the technical foundations for the extension of the Topology ToolKit (TTK) to distributed-memory parallelism with the Message Passing Interface (MPI). While several recent papers introduced topology-based approaches for distributed-memory environments, these were reporting experiments obtained with tailored, mono-algorithm implementations. In contrast, we describe in this paper a versatile approach (supporting both triangulated domains and regular grids) for the support of topological analysis pipelines, i.e. a sequence of topological algorithms interacting together. While developing this extension, we faced several algorithmic and software engineering challenges, which we document in this paper. We describe an MPI extension of TTK's data structure for triangulation representation and traversal, a central component to the global performance and generality of TTK's topological implementations. We also introduce an intermediate interface between TTK and MPI, both at the global pipeline level, and at the fine-grain algorithmic level. We provide a taxonomy for the distributed-memory topological algorithms supported by TTK, depending on their communication needs and provide examples of hybrid MPI+thread parallelizations. Performance analyses show that parallel efficiencies range from 20% to 80% (depending on the algorithms), and that the MPI-specific preconditioning introduced by our framework induces a negligible computation time overhead. We illustrate the new distributed-memory capabilities of TTK with an example of advanced analysis pipeline, combining multiple algorithms, run on the largest publicly available dataset we have found (120 billion vertices) on a cluster with 64 nodes (for a total of 1536 cores). Finally, we provide a roadmap for the completion of TTK's MPI extension, along with generic recommendations for each algorithm communication category.

==> sharedVersusDistributed.tex <==
\begin{figure}
  \centering

\includegraphics[width=\linewidth]{figures/plot_multiple_strong_exec_time_comp.pdf}
  \caption{\majorRevision{
  Comparing TTK's shared-memory-only parallelism ($1 \times 24$: 1 process, 24 threads) with two instances of our novel distributed-memory parallelism support: MPI+thread ($2\times12$: 2 processes, 12 threads per process) and pure MPI ($24\times1$: 24 processes, 1 thread per process) for the algorithms of
%   \autoref{sec_background}
  Sec. 2
  on a single compute node.}}
%   ($2\times12$: 2 processes, 12 threads per process and $24\times1$: 24 processes, 1 thread per process)
%   Performance results of different configuration for an
%   execution on one node.}}
  \label{fig_sharedVSdistributed}
\end{figure}

\section{\major{Shared VS distributed parallelism}}
\label{sec_comparisonSharedVSdistributed}
\major{In this section, we evaluate the performance of our novel support for distributed-memory parallelism, in comparison to TTK's
% pre-existing
% sole
shared-memory-only parallelism. For this,
to reach a common ground,
we restrict the experiments on a single compute node. Moreover, we resample the input datasets to $512^3$ (via trilinear interpolation) to reach a sufficient workload.
\autoref{fig_sharedVSdistributed} reports the execution time of
% Next, we analyze the execution time of
the algorithms presented in
% \autoref{sec_background}
Sec. 2
with several strategies:
TTK's
% pre-existing
shared-memory-only
parallelism, modeled here by a 1 x 24 configuration (1 process, 24 threads), our novel support for an MPI+thread strategy ($2 \times 12$: 2 processes, 12 threads per process) as well as our novel support for a pure MPI strategy ($24 \times 1$: 24 processes, 1 thread per process).
For the embarrassingly parallel algorithms (\emph{ScalarFieldCriticalPoints, DiscreteGradient}) belonging to the \emph{No Communication (NC)} category
% (\autoref{sec_taxonomy}),
(Sec. 6.1),
performances are nearly identical for the three strategies, which confirms that our novel framework for distributed computations in TTK does not impact negatively the performances of these algorithms, in comparison to TTK's
% pre-existing
shared-memory-only parallelism. For the algorithms belonging to the other categories, and which require inter-process communications, performances necessarily start to decrease, as communications induce inter-process synchronizations, which degrade parallel efficiency. This is illustrated with the algorithm \emph{ScalarFieldSmoother}.
% Note that, while it induces more inter-process communications, shifting from $2$ processes to $24$ still results in nearly identical performances, which indicates
% efficient communications
% that the communication costs are not significant with regard to the rest of the computation.
% Finally, i
Interestingly,
% although the algorithm \emph{IntegralLines} does require communications, its
the
performances of the algorithm \emph{IntegralLines} in MPI+thread mode ($2\times12$) are significantly improved over a pure MPI strategy ($24 \times 1$),
hence highlighting the advantages in terms of workload sharing of the MPI+thread strategy. Thanks to this,
if we exclude the stress datasets (\emph{Elevation} and \emph{Random}, which are synthetic worst cases),
the performances of the algorithm \emph{IntegralLines} in distributed mode (MPI+thread strategy, $2\times12$) are nearly identical to that of the shared-memory-only parallel implementation ($1\times 24$, processing seeds in parallel, as described in
Sec. 6.3.5).}
% \autoref{sec_integralLines}).}

\major{Overall, \autoref{fig_sharedVSdistributed} also shows that, on a single compute node, the best performances are obtained
by using one MPI process and using a number of threads equal to the number of available cores.
% on the compute node.
As discussed in Sec. 7.1.1, this leads to an improved memory footprint (fewer ghost simplices are necessary) and hence, fewer MPI communications and synchronizations. Thus, for our MPI+thread strategy, we systematically rely on one MPI process per node (and 24 threads within).}

\major{In conclusion, our novel framework for distributed computations in TTK
enables the processing of significantly larger datasets (as documented
in Sec. 6.4)
% \autoref{sec_integratedPipeline})
than TTK's pre-existing shared-memory-only parallelism, while resulting in similar runtime performances for
most of
the considered algorithms
%
% provides similar runtime performances to TTK's pre-existing shared-memory parallelism for most algorithms
(\emph{ScalarFieldCriticalPoints}, \emph{DiscreteGradient}, and \emph{IntegralLines}).
Parallel efficiency
% does
decreases for \emph{ScalarFieldSmoother}, as it
% at the exception of \emph{ScalarFieldSmoother}, which
requires inter-process synchronizations.
% (hence decreasing parallel efficiency).
% Moreover,
Also,
as shown for \emph{IntegralLines}, our MPI+thread strategy significantly improves runtime performances in comparison to a pure MPI strategy.}

